Unified Perception: Efficient Depth-Aware Video Panoptic Segmentation with Minimal Annotation Costs

Depth-aware video panoptic segmentation is a promising approach to camera based scene understanding. However, the current state-of-the-art methods require costly video annotations and use a complex training pipeline compared to their image-based equivalents. In this paper, we present a new approach titled Unified Perception that achieves state-of-the-art performance without requiring video-based training. Our method employs a simple two-stage cascaded tracking algorithm that (re)uses object embeddings computed in an image-based network. Experimental results on the Cityscapes-DVPS dataset demonstrate that our method achieves an overall DVPQ of 57.1, surpassing state-of-the-art methods. Furthermore, we show that our tracking strategies are effective for long-term object association on KITTI-STEP, achieving an STQ of 59.1 which exceeded the performance of state-of-the-art methods that employ the same backbone network. Code is available at: https://tue-mps.github.io/unipercept

==> figures/styles.tex <==
\makeatletter

% Typography
\tikzset{
    font={\small}
}

% Module related styles
\tikzset{
    module/.style={rounded corners, draw=black!40, fill=black!1, thick, minimum size=12mm, text width=20mm, align=center},
    loss/.style={rounded corners, draw=yellow!50, fill=yellow!20, very thick, minimum size=5mm},
    op/.style={circle, draw=black!60, fill=black!2, thick, minimum size=1mm, inner sep=0.5mm},
    data/.style={rectangle, very thick, inner sep=2mm, align=center, draw=blue!20, fill=blue!2}
}

% Image style
\tikzset{
    image/.style={rectangle, inner sep=0, align=center}
}

% Region
\tikzset{
    region/.style={rounded corners, dotted, thick, inner sep=3mm, draw=black!60, align=left}
}

% Database
\tikzset{
    database/.style={
            path picture={
                    \draw (0, 1.5*\database@segmentheight) circle [x radius=\database@radius,y radius=\database@aspectratio*\database@radius];
                    \draw (-\database@radius, 0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
                    \draw (-\database@radius,-0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
                    \draw (-\database@radius,1.5*\database@segmentheight) -- ++(0,-3*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius] -- ++(0,3*\database@segmentheight);
                },
            minimum width=2*\database@radius + \pgflinewidth,
            minimum height=3*\database@segmentheight + 2*\database@aspectratio*\database@radius + \pgflinewidth,
        },
    database segment height/.store in=\database@segmentheight,
    database radius/.store in=\database@radius,
    database aspect ratio/.store in=\database@aspectratio,
    database segment height=0.1cm,
    database radius=0.25cm,
    database aspect ratio=0.35,
}

\makeatother
